Comprehensive Library of Variational LSE Solvers

Linear systems of equations can be found in various mathematical domains, as well as in the field of machine learning. By employing noisy intermediate-scale quantum devices, variational solvers promise to accelerate finding solutions for large systems. Although there is a wealth of theoretical research on these algorithms, only fragmentary implementations exist. To fill this gap, we have developed the variational-lse-solver framework, which realizes existing approaches in literature, and introduces several enhancements. The user-friendly interface is designed for researchers that work at the abstraction level of identifying and developing end-to-end applications.

==> figures/experiment_old.tex <==
\begin{figure}[t]
    % \pgfplotsset{colormap/jet}
    \centering

\subfigure[Training loss for $100$ random initializations, variance in pale colors.]{
\begin{tikzpicture}
        \centering
        \begin{axis}[
            name=plot1,
            xlabel=$\textbf{step}$,
            ylabel=$\textbf{loss}$,
            ymode=log,
            % xtick={1, 3, 5, 7, 9, 11},
            % ytick={0, 10, 200, 300, 400, 500},
            % xtick={0, 10, 20, 30, 40},
            xmin=0,xmax=51.5,
            ymin=0.0005,ymax=1.5,
            ytick={1.0, 0.1, 0.01, 0.001},
            yticklabels={,$10^{-1}$,$10^{-2}$,$10^{-3}$},
            % restrict y to domain=0.0:500.0,
            label style={font=\footnotesize},
            tick label style={font=\footnotesize},
            % grid=y,
            ymajorgrids=true,
            axis x line=bottom, axis y line=left,
            width=0.7\linewidth,
            height=3cm,
            legend style={/tikz/every even column/.append style={column sep=0.1cm, row sep=0.1cm},at={(1.55,0.65)},anchor=east,yshift=-5mm,font=\scriptsize}]
            ]

             % \legend{,,,\texttt{qtm} ~~($\alpha_{\boldsymbol{\theta}} = 0.01\text{, }~\alpha_{\boldsymbol{\lambda}} = 0.1$),,,,\texttt{qml-rev} ~~($\alpha_{\boldsymbol{\theta}} = \alpha_{\boldsymbol{\lambda}} = 0.05$)}

             \legend{,,,\texttt{global},,,,\texttt{local}, groud truth}
            
            % Global loss
            \addplot+[draw=none,name path=A,no markers] %
            	table[x=step,y=loss_std_upper,col sep=comma]{figures/data/train_global_fun.csv};
            \addplot+[draw=none,name path=B,no markers] %
            	table[x=step,y=loss_std_lower,col sep=comma]{figures/data/train_global_fun.csv};
            \addplot[color_global!40] fill between[of=A and B];
            \addplot[line width=.7pt,solid,color=color_global] %
            	table[x=step,y=loss_avg,col sep=comma]{figures/data/train_global_fun.csv};

            % Local loss
            \addplot+[draw=none,name path=A,no markers] %
            	table[x=step,y=loss_std_upper,col sep=comma]{figures/data/train_local.csv};
            \addplot+[draw=none,name path=B,no markers] %
            	table[x=step,y=loss_std_lower,col sep=comma]{figures/data/train_local.csv};
            \addplot[color_local!40] fill between[of=A and B];
            \addplot[line width=.7pt,solid,color=color_local] %
            	table[x=step,y=loss_avg,col sep=comma]{figures/data/train_local.csv};

            \addplot[color=color_classical, domain=0.0:0.001, line width=.7pt] {0.001};

        \end{axis}
        \end{tikzpicture}
    }
    \\
    \subfigure[Evaluated result compared to normalized classical solution, error bars show $25$th and $75$th percentiles over the $100$ trained parameter sets.]{
        \begin{tikzpicture}
            \begin{axis}[
            name=plot2,
            width=0.99\linewidth, height=3cm,
            ymajorgrids,
            label style={font=\footnotesize},
            tick label style={font=\footnotesize},
            xmin=-.5,xmax=7.5,
            ymin=0,ymax=0.21,
            xtick={0, 1, 2, 3, 4, 5, 6, 7},
            xticklabels={000, 001, 010, 011, 100, 101, 110, 111},
            ytick={0.0,0.1,0.2},
            ylabel=$\textbf{value}$,
            ybar = .05cm,
            bar width = 5.5pt,
            axis x line=bottom, axis y line=left, tick align = outside,
            x axis line style = {-},
            legend columns=-1,
            legend style={/tikz/every even column/.append style={column sep=0.1cm},at={(0.6,0.8)},anchor=south,yshift=-5mm}, 
            ]
            \addplot[fill=color_classical!90,ybar,no marks,error bars/.cd, y dir=both, y explicit] coordinates {
                (0,0.084)
                (1,0.084)
                (2,0.166)
                (3,0.166)
                (4,0.084)
                (5,0.084)
                (6,0.166)
                (7,0.166)
            };

            \addplot[fill=color_global!80,ybar,no marks,error bars/.cd, y dir=both, y explicit] coordinates {
                (0,0.086) +- (0.007,0.009)
                (1,0.083) +- (0.007,0.011)
                (2,0.165) +- (0.012,0.013)
                (3,0.159) +- (0.011,0.010)
                (4,0.088) +- (0.009,0.008)
                (5,0.085) +- (0.007,0.009)
                (6,0.171) +- (0.009,0.010)
                (7,0.163) +- (0.009,0.009)
            };

            \addplot[fill=color_local!80,ybar,no marks,error bars/.cd, y dir=both, y explicit] coordinates {
                (0,0.083) +- (0.008,0.008)
                (1,0.084) +- (0.007,0.007)
                (2,0.162) +- (0.010,0.009)
                (3,0.166) +- (0.008,0.010)
                (4,0.087) +- (0.009,0.007)
                (5,0.084) +- (0.007,0.007)
                (6,0.166) +- (0.010,0.010)
                (7,0.167) +- (0.010,0.011)
            };

        \end{axis}
        \end{tikzpicture}
        \label{subfig:spectrum}
    }
    
    \caption{\label{fig:exp}Results produced with the proposed framework on the \gls{lse} described in~\cref{eq:lse_1,eq:lse_2}. The variational ansatz consists of a depth $d=1$ version of~\cref{fig:circuit}. The training for $50$ steps in (a) shows smooth convergence for both loss functions. The evaluation of the final results with $1000$ shots in (b) is in good agreement with the classical solution.}
\end{figure}
